Dynamic Mortality Risk Predictions in Pediatric Critical Care Using Recurrent Neural Networks

Viewing the trajectory of a patient as a dynamical system, a recurrent neural network was developed to learn the course of patient encounters in the Pediatric Intensive Care Unit (PICU) of a major tertiary care center. Data extracted from Electronic Medical Records (EMR) of about 12000 patients who were admitted to the PICU over a period of more than 10 years were leveraged. The RNN model ingests a sequence of measurements which include physiologic observations, laboratory results, administered drugs and interventions, and generates temporally dynamic predictions for in-ICU mortality at user-specified times. The RNN's ICU mortality predictions offer significant improvements over those from two clinically-used scores and static machine learning algorithms.

==> drtedv2_section_cnn.tex <==
\section{CNN-based Framework}

%The goal of the CNN framework is to generate a data structure from the unstructured EMR data in order to predict the probability of survival for a patient from the first 12 hours of data available from an ICU encounter. Significant effort went into generating a data structure which could be readily ingested into a pre-existing deep learning framework \citep{keras2015}.  This was accomplished through the creation of a 'Patient Snapshot' which is described in section \ref{sub:patientsnapshot}. This 'image' representation enables utilization of state-of-the-art algorithms which have been developed in the computer vision field over the past several years \citep{krizhevsky2012imagenet, simonyan2014very, szegedy2015going,he2015deep}.
We developed a CNN framework to predict the probability of survival of a patient from the first 12 hours of ICU encounter.  To leverage state-of-the-art algorithms from the computer vision field \citep{krizhevsky2012imagenet, simonyan2014very, szegedy2015going,he2015deep}, we first had to convert the unstructured EMR into a data structure that can be readily ingested by these algorithms.  This section discusses that data structure. 

%This was accomplished through the creation of a 'Patient Snapshot' which is described in section \ref{sub:patientsnapshot}. 

%\subsection{Patient Snapshot}
%\label{sub:patientsnapshot}
%After scrubbing, a patient record contains a vector of values with each vector element corresponding to a particular variable at a particular time.  The goal of the matrix representation is to pivot that data into an image representation which can be utilized by a CNN. In order to accomplish this task the data is re-sampled at a regular interval (nominally 5 minutes). A simple forward fill imputation is utilized to fill any missing data. While not the most advanced imputation method, a forward fill imputation is a reasonable assumption for medical data where it is assumed that when nothing is changing (i.e. patient is stable), then either very sparse or no new measurements need be taken; and when a precipitous event occurs, new measurements are taken at a much higher frequency.
After pre-processing, a patient encounter record contains a vector wherein a single element corresponds to a measurement of a particular variable at a particular time. This vector is transformed to a matrix, where each row of entries corresponds to the time series of one of the 173 variables in the dataset.  A single column reflects the patient at one point in time, and the columns are regularly-spaced (nominally 5 minutes). Therefore,  
all the variables are re-sampled on this regular temporal grid.  A simple forward fill imputation is utilized to fill any missing data. While other imputation techniques are available, a forward fill imputation is a reasonable choice based on the assumption that new measurements are sparsely taken when the patient appears stable but more frequently when a precipitous event occurs.  We refer to these matrix representations of patients as {\it{Patient Snapshots}}. Figure \ref{fig:patient_snapshots} illustrates two examples.

%Once the data has been re-sampled at a regular frequency, a simple pivot operation generates the desired data structure in which the matrix rows represent each available variable and the columns represent the temporal dimension of the data. Depending on the encounter length of the patient, this matrix can be trimmed to the appropriate number of elements on the X-axis (nominally 144 for a 12-hour encounter with 5-minute sampling).


\begin{figure}[htbp]
  \centering 
  \includegraphics[scale=0.55]{Figures/HighProv_vs_LowProb_PatientSnapshots_1_.eps} 
  \caption{Two examples of patient snapshots with laboratory measurements, vitals, drugs, and interventions along the y-axis and time along the x-axis. The 144 columns are 5 minutes apart, so that each snapshot captures 12 hours of ICU data.  On the left is a snapshot from a patient who was alive at the end of the ICU encounter, while on the right is from a patient who died. Higher volatility in the non-surviving patient is clearly visible.}
  \label{fig:patient_snapshots} 
\end{figure} 

Since we {\it{artificially}} construct the patient snapshots, there are certain relationships within them that we understand and exploit.  For example, we utilize 1-D convolutions along the rows to extract temporal trends within each variable.  Communications between the variables occur in dense layers after the 1-D convolutions.  A re-ordering of the rows to leverage known correlations between particular variables with 2-D convolutions is a direction for further inquiry.  The complete architecture for the PICU data is in Appendix B, Figure \ref{fig:cnn_model}.
   
%Since we understand that the relationships in the patient snapshot are structured in a specific format, unlike naturally imagery, we are able to specifically exploit the temporal relationships via 1-D convolutions. The complete architecture can be seen in Figure \ref{fig:cnn_model} in Appendix B.

